Combining high contrast imaging and radial velocities to constrain the planetary architecture of nearby stars

Nearby stars are prime targets for exoplanet searches and characterization using a variety of detection techniques. Combining constraints from the complementary detection methods of high contrast imaging (HCI) and radial velocity (RV) can further constrain the planetary architectures of these systems because these methods place limits at different regions of the companion mass and semi-major axis parameter space. We aim to constrain the planetary architectures from the combination of HCI and RV data for 6 nearby stars within 6 pc: $\tau$ Ceti, Kapteyn's star, AX Mic, 40 Eri, HD 36395, and HD 42581. We compiled the sample from stars with available archival VLT/NACO HCI data at L$^{\prime}$ band (3.8 $\mu$m). The NACO data were fully reanalyzed using the state-of-the-art direct imaging pipeline PynPoint and combined with RV data from HARPS, Keck/HIRES, and CORALIE. A Monte Carlo approach was used to assess the completeness in the companion mass/semi-major axis parameter space from the combination of the HCI and RV data sets. We find that the HCI data add significant information to the RV constraints, increasing the completeness for certain companions masses/semi-major axes by up to 68 - 99% for 4 of the 6 stars in our sample, and by up to 1 - 13% for the remaining stars. The improvements are strongest for intermediate semi-major axes (15 - 40 AU), corresponding to the semi-major axes of the ice giants in our own solar system. The HCI mass limits reach 5 - 20 $M_{\textrm{Jup}}$ in the background-limited regime, depending on the age of the star. Through the combination of HCI and RV data, we find that stringent constraints can be placed on the possible substellar companions in these systems. Applying these methods systematically to nearby stars will quantify our current knowledge of the planet population in the solar neighborhood and inform future observations.

==> NACO_obs_aa.tex <==
\begin{table*}[]
    \caption{Summary of Archival NACO Imaging Observations}
    \label{tab:NACO_obs}
    \centering
\begin{tabular}{lcccccc}
\hline \hline
% \tablehead{
%   \colhead{Star} & 
%   \colhead{Date} & 
%   \colhead{On-source $t_{\text{int}}$} & 
%   \colhead{\# of frames} & 
%   \colhead{Airmass} & 
%   \colhead{Field rotation} & 
%   \colhead{Program ID} \\ 
% % 
% % 
%   \colhead{} & 
%   \colhead{(UT)} & 
%   \colhead{(minutes)} & 
%   \colhead{} & 
%   \colhead{} & 
%   \colhead{(deg)} & 
%   \colhead{} 
% }

Star & Date & On-source $t_{\text{int}}$ &  \# of frames &  Airmass &   Field rotation &   Program ID \\ 
  & (UT) & (minutes) &  &  &  & \\
\hline
tau Ceti & 2008-11-16 & 12 & 4137 & 1.02 - 1.07 & 19 & 082.C-0518 \\ 
Kapteyn's star & 2008-11-16 & 23 & 2815 & 1.10 - 1.14 & 15 & 082.C-0518 \\ 
AX mic & 2009-10-11 & 10 & 3423 & 1.07 - 1.12 & 14 & 084.C-0656 \\ 
40 Eri & 2008-11-16 & 11 & 1268 & 1.05 - 1.07 & 21 & 082.C-0518 \\ 
HD 36395 & 2008-11-16 & 19 & 3842 & 1.08 - 1.12 & 18 & 082.C-0518 \\ 
HD 42581 & 2008-11-16 & 19 & 3723 & 1.00 - 1.01 & 53 & 082.C-0518 \\ 

\hline

\end{tabular}
\end{table*}
